Generalizations of Guillera-Sondow's double integral formulas

We evaluate certain multidimensional integrals in terms of the Lerch transcendent function $\Phi$, generalizing Guillera-Sondow's formulas. As an application, we get new representations of classical constants like Euler's constant $\gamma$ and $\ln(4/\pi)$.

==> Garbage.tex <==
\begin{theorem}
If either $z \in \C - [1, \infty)$ and $\Re(s)>-3$, or $z=1$
and $\Re(s)>-2$, then
\begin{multline*} 
\int_{\cube{m}} \frac{m-1 - x_1-x_1 x_2 - \cdots - x_1 x_2 \cdots x_{m-1}}
{1-z x_1 x_2 \cdots x_m} (x_1 x_2 \cdots x_m)^{u-1}
(-\ln x_1 x_2 \cdots x_m)^{s-m+2} \, d \overline x
\\ = \frac{\Gamma(s+2)}{(m-2)!} \left[ \Phi(z,s+2,u)+\frac{(1-z)
\Phi(z,s+1,u)-u^{-s-1}}{z (s+1)} \right].
\end{multline*}
\end{theorem}

